Dealing with Controversy: An Emotion and Coping Strategy Corpus Based on Role Playing

There is a mismatch between psychological and computational studies on emotions. Psychological research aims at explaining and documenting internal mechanisms of these phenomena, while computational work often simplifies them into labels. Many emotion fundamentals remain under-explored in natural language processing, particularly how emotions develop and how people cope with them. To help reduce this gap, we follow theories on coping, and treat emotions as strategies to cope with salient situations (i.e., how people deal with emotion-eliciting events). This approach allows us to investigate the link between emotions and behavior, which also emerges in language. We introduce the task of coping identification, together with a corpus to do so, constructed via role-playing. We find that coping strategies realize in text even though they are challenging to recognize, both for humans and automatic systems trained and prompted on the same task. We thus open up a promising research direction to enhance the capability of models to better capture emotion mechanisms from text.

==> Supplementary_material/Pre-test/descriptions-pretest-round1.tex <==
\begin{table*}
    \begin{tabularx}{\textwidth}{p{2cm}p{12.5cm}}
\toprule
\textbf{Strategy} & \textbf{Description}\\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Attack & X does not shy away from unpleasant situations. When things are bad, X  invests significant effort in understanding why. Why did they go that way? This character is inclined to identify causes of discomfort, to confront them head-on, and attempt to rectify their consequences. That is when one can see X all tense and pumped up, committed to overcome an obstacle hindering a better life.

Injustice hurts X profoundly. This character affirms what bothers it by facing the source of stress directly and aggressively. Always ready to right the wrong, X takes action to change the situation, and can come across as attacking. But this severity does not only apply to others: if X is responsible for their failures or something wrong, X reproaches itself.\\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Contact & This character possesses a constructive, problem-solving mindset. X expresses ideas and desires with confidence, striving to achieve practical objectives. X understands the importance of self-worth.

For X, communication serves to unite people. It is an opportunity to exchange opinions openly and respectfully, acknowledging the diversity of perspectives among individuals. X can effectively engage in discussions also with people holding contrasting opinions. 

X maintains this attitude even in the context of unpleasant situations: X engages with the source of stress in a proactive manner, coming across as a very approachable person.\\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Distance & This character is avoidant. Unpleasant events make X feel powerless, as if the potential repercussions were entirely uncontrollable. X thinks there's not much one can do to change the external world. One can act on oneself, though.

For X, tense, confrontational exchanges with other people are not a source of excitement. Accompanied by a sense of anxiety, this person has developed a strong defence strategy to deflect focus from stressful things, events, people or thoughts: keeping oneself away from all wrongdoings (both personal and of others). Conflicts and uncomfortable situations should be avoided at all costs, with the effort to minimise their negative influence in one's life. \\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Reject & ``No time for fools, it's best to keep one's distance from other people''. This is a typical way of thinking of X, a person who does not easily approach or trust others. X believes that nobody can get an important job done: it's best to work and be alone, even if that creates some distance with the rest of the world.

This person is prone to being displeased, ready to wrinkle in aversion. X would really prefer not to be involved in any difficult situation. In fact, X withdraws from any circumstance mismatching personal goals or preferences, and tries to minimise the engagement with the cause of such distress. This character tends to deny the influence of unpleasant, negative things. If there were one motto in life, X's would be: bring yourself in a state of peace.\\
\bottomrule
\end{tabularx}
\caption{Descriptions used in the pre-test, for Round 1.}
\label{pre-study-descriptions-1}
\end{table*}

==> Supplementary_material/Pre-test/descriptions-pretest-round2.tex <==
\begin{table*}
    \begin{tabularx}{\textwidth}{p{2cm}p{12.5cm}}
\toprule
\textbf{Strategy} & \textbf{Description}\\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Attack & When unpleasant situations arise, X responds with a hardened resolve. This character does not seek consolation or advice from others, but instead confronts problems head-on, often with an aggressive and intense energy. X's approach to overcoming obstacles is a solo fight to right the wrong.

Injustice hurts X profoundly; unfairness is a trigger, igniting a spark that pushes this character to face the source of stress directly and fiercely. Why did things go that way? X is driven to identify the causes of discomfort, to confront them head-on, in the attempt to rectify their consequences.

X, who does not shy away from conflicts, takes action to change negative situations in a proactive manner, and can come across as combative. That is when one can see X all tense and pumped up, committed to overcome an obstacle. This resolution isn't only aimed outwards; if X perceives personal failure or wrongdoing, it has a tendency to self-criticize and demand more. \\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Reject & This person, who does not easily trust others, is prone to being displeased, always ready to wrinkle in aversion. So here's how X approaches life: the world is simpler when one refuses to engage in negativity. A striking characteristic of X is this ability to deflect interactions that could result in conflict. One could almost say that unpleasant events do not concern X's existence, because X has mastered the skill of rebuking circumstances that mismatch personal goals or preferences.

When faced with a source of potential distress, X effectively minimizes its importance or impact. This is not due to a lack of courage, but to a fundamental belief that it's better to completely repudiate all difficulties. For this character, personal tranquility rules above all else, and uncomfortable situations must be dismissed at all costs. \\

\bottomrule
\end{tabularx}
\caption{Descriptions used in the pre-test, for Round 2.}
\label{pre-study-descriptions-2}
\end{table*}

==> Supplementary_material/Pre-test/descriptions-pretest-round3.tex <==
\begin{table*}
    \begin{tabularx}{\textwidth}{p{2cm}p{12.5cm}}
\toprule
\textbf{Strategy} & \textbf{Description}\\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Attack & When unpleasant situations arise, X responds with a hardened resolve. This character confronts problems head-on, often with an aggressive and intense energy. X's approach to overcoming obstacles is a solo fight to right the wrong.

Unfairness is a trigger for X, igniting a spark that pushes this character to fight the source of stress fiercely. Why did things go that way? X does not shy away from conflicts, and tries to identify the causes of discomfort in the attempt to rectify their consequences.

X takes action to change negative situations personally. For this reason, X can come across as combative. One can often see X tense and pumped up, committed to overcome an obstacle. This resolution isn't only aimed outwards; if X perceives personal failure or wrongdoing, it has a tendency to self-criticize and demand more. \\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Contact & This character possesses a constructive, problem-solving mindset. X expresses ideas and desires with confidence, striving to achieve practical objectives. X understands the importance of self-worth.

For X, communication serves to unite people. It is an opportunity to exchange opinions openly and respectfully, acknowledging the diversity of perspectives among individuals. X can effectively engage in discussions also with people holding contrasting opinions. 

X maintains this attitude even in the context of unpleasant situations: X engages with the source of stress in a proactive manner, coming across as a very approachable person.\\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Distance & This character is avoidant. Unpleasant events make X feel powerless, as if the potential repercussions were entirely uncontrollable. X thinks there's not much one can do to change the external world. One can act on oneself, though: rather than engaging in conflict or confrontations, X seeks emotional and mental space, finding solace in self-reflection.

For X, tense, confrontational exchanges with other people are not a source of excitement. Accompanied by a sense of anxiety, this person has developed a strong defense strategy to deflect focus from stressful things, events, people or thoughts: keeping oneself away from all wrongdoings (both personal and of others). Conflicts and uncomfortable situations should be avoided at all costs, with the effort to minimize their negative influence in one's life. \\
\cmidrule(r){1-1}\cmidrule(r){2-2}
Reject & This person easily disagrees with others, and has a quite judgmental attitude towards their behaviors and beliefs. For this reason X is often displeased, ready to wrinkle in aversion when people don't align with X's expectations.

For this character, uncomfortable situations must be dismissed at all costs. So here's X's approach to life: just let people with ideas that you dislike not interfere with your personal well-being -- not by aggressively facing them, but confidently let them know your position.

X tends to refuse negativity: all circumstances that mismatch personal goals or preferences can be turned down, not due to a lack of courage, but to a fundamental belief that it's better to solve difficulties by directly getting rid of them.\\
\bottomrule
\end{tabularx}
\caption{Descriptions used in the pre-test, for Round 3.}
\label{tab:pre-study-descriptions-3}
\end{table*}

==> Supplementary_material/Pre-test/descriptions-pretest-round4.tex <==
\begin{table*}
\centering
\begin{tabular}{p{14cm}p{2cm}}
\toprule
\multicolumn{2}{c}{\textbf{Strategy: Attack}}\\
\cmidrule(r){1-2}
\textbf{Description}: X is a very opinionated person, who comes across as aggressive and combative.
When problems or unpleasant situations arise, X responds with a hardened resolve. X gives their all to overcome obstacles, and never shies away from a conflict. In fact, this character faces negative situations fiercely and with intense energy, taking action personally in order to right the wrong. For this reason, one can often see X all tense and pumped up.&\multirow{2}{*}{\includegraphics[scale=.25]{figs/pre-test/sketches/VisualCopingStrat-Attacking.png}}\\

\textbf{Short summary}: X rights the wrong in an aggressive manner, like in the picture below (X is shown in blue). &\\\\

\midrule
\multicolumn{2}{c}{\textbf{Strategy: Contact}}\\
\cmidrule(r){1-2}
{\bf Description}: This character comes across as a calm, understanding, and very approachable person. For X, communication serves to unite people. It is an opportunity to exchange opinions, acknowledging the diversity of perspectives among individuals. When problems or unpleasant situations arise, this character responds with a constructive attitude. X expresses ideas with confidence, trying to solve problems in a respectful manner. X can effectively engage in discussions also with people having contrasting opinions.&\multirow{2}{*}{\includegraphics[scale=.25]{figs/pre-test/sketches/VisualCopingStrat-Contacting.png}}\\

\textbf{Short summary}:  X rights the wrong with an open mindset, like in the picture below (X is shown in blue).&\\\\\\[.5pt]

\midrule
\multicolumn{2}{c}{\textbf{Strategy: Distance}}\\
\cmidrule(r){1-2}
\textbf{Description}: In life, X has managed to create a peaceful mental space as a protection from the outside world. This character always seeks emotional tranquillity, and finds solace in self-reflection. When problems or unpleasant situations arise, X feels powerless, not too capable to change the external world. So here's X's defense strategy against all negativity: staying away from stressful things, events, people or thoughts, to minimize their influence. At the cost of coming across as an avoidant person, X does not engage in conflicts and uncomfortable situations. & \multirow{2}{*}{\includegraphics[scale=.25]{figs/pre-test/sketches/VisualCopingStrat-Distancing.png}}\\

\textbf{Short summary}: X seeks shelter from unpleasant situations in a quiet inner space, like in the picture below
(X is shown in blue).&\\\\[.5pt]

\midrule
\multicolumn{2}{c}{\textbf{Strategy: Reject}}\\
\cmidrule(r){1-2}

\textbf{Description}: This person has a judgmental attitude towards others. X easily disagrees with people, and is often displeased with their behaviors and beliefs. Here's X’s motto in life: do not let anybody interfere with your well-being. This character keeps negativity away at all costs. It's not that X hides from problems and tries to find solace in a peaceful mental space, it's more of a resolute attempt to refuse unpleasant situations. It's also not a lack of courage; in fact, X expresses opinions with confidence, and precisely by this, X manages to dismiss conflicts with other people. & \multirow{2}{*}{\includegraphics[scale=.25]{figs/pre-test/sketches/VisualCopingStrat-Rejecting.png}}\\

\textbf{Short summary}: 
X's approach to life is a firm refusal of negativity, like in the picture below
(X is shown in blue). &
\\\\

\bottomrule
\end{tabular}
\caption{Descriptions of $X$ used in the final round of coping recognition and in the role-playing crowdsourcing phase. Each copying strategy is presented as a description of character $X$, and in a more concise version (short summary), and with the reported picture.}
\label{tab:pre-study-descriptions-4}
\end{table*}

==> Supplementary_material/Scenarios/Slim-scenarios.tex <==
\onecolumn
{\small
\begin{longtable}{p{16cm}}
\caption{ChatGPT-4 generation of scenarios. Green rows correspond to humans, white rows to the assistant's replies. For simplicity, we only report one generated scenario.}\label{tab:scenarios-chat} \\
\toprule
\rowcolor{lightgreen}
I am conducting a study about Roseman's coping strategies (i.e., attack, contact, distance and reject). My goal is to study how each strategy realises in language when speakers discuss about controversial topics. Imagine that during an interaction, one of the interlocutors expresses an opinion that makes another uncomfortable; the latter thus responds with a verbal utterance and a non-verbal reaction while being "under the influence" of a coping strategy.\\

Certainly! Studying how Roseman's coping strategies manifest in language, especially during discussions on controversial topics, is an intriguing area of inquiry. When individuals discuss controversial topics and face conflicting or uncomfortable opinions, they might adopt one or more of Roseman's coping strategies in their verbal and non-verbal behavior.

Here's a breakdown of each strategy along with potential verbal and non-verbal manifestations:\\
1.  {\bf Attack}:

{\bf Verbal}: An individual might use aggressive language, accusations, or challenges. They might say things like, "That's completely wrong," "How can you even believe that?", or "You clearly haven't done your research." 

{\bf Non-Verbal}: Physically leaning forward, intense eye contact, clenched fists, raised voice, or even pointing fingers. The individual's face might show signs of anger or frustration.\\

2.  {\bf Contact}:
    
   {\bf Verbal}: The individual would seek clarification, ask questions, or try to understand the other's viewpoint. They might say, "Can you explain why you feel that way?", "I'm curious to know more about your perspective," or "Let's find some common ground."
    
    {\bf Non-Verbal}: Leaning in, maintaining steady but non-threatening eye contact, nodding to indicate active listening, and open body posture. The face might reflect genuine curiosity or concern.\\

3.  {\bf DISTANCE}:
    
     {\bf Verbal}: An individual might divert the topic, use vague language, or minimize their involvement in the conversation. They might say, "Let's discuss this later," "I need some time to think about it," or simply change the topic altogether.
     
   {\bf Non-Verbal}: Looking away, physically leaning back, creating physical distance, crossing arms as a defensive posture, or checking one's phone/watch. The face might show signs of discomfort or avoidance.\\

4.  {\bf Reject}:
    
    {\bf Verbal}: The individual might dismiss the topic or the person's opinion outright, often without offering a counter-argument. They might say, "That's not even worth discussing," "I can't entertain that thought," or "We'll never agree on this, so let's drop it."
    
    {\bf Non-Verbal}: Eye-rolling, shaking the head, waving one's hand dismissively, or even walking away. The face might display contempt, disdain, or indifference.\\
  

For a comprehensive study, you may also want to consider the tone of voice, the specific linguistic constructions used, the rhythm and pace of speech, and other nuanced non-verbal cues like pupil dilation or micro-expressions. Moreover, always remember that cultural and individual variations can affect how these coping strategies manifest. It would be beneficial to take these variations into account when analyzing and interpreting your findings.\\\\

\rowcolor{lightgreen}
With my next prompts, I'm going to ask you to conduct the following task. 

{\bf Task} Depict three scenarios (each set in a different social context, briefly described) in which two characters, X and Y, interact. Y produces a controversial statement about a given topic that I will specify. That opinion could elicit an emotional reaction in X. Each scenario must be structured like so: 

- SCENARIO AND CONTROVERSIAL OPINION 

- VERBALIZED REACTION AND NON VERBALIZED REACTION ASSUMING THAT PERSON B ADOPTS THE COPING STRATEGY OF ATTACK 

- VERBALIZED REACTION AND NON VERBALIZED REACTION ASSUMING THAT PERSON B ADOPTS THE COPING STRATEGY OF CONTACT 

- VERBALIZED REACTION AND NON VERBALIZED REACTION ASSUMING THAT PERSON B ADOPTS THE COPING STRATEGY OF DISTANCE - VERBALIZED REACTION AND NON VERBALIZED REACTION ASSUMING THAT PERSON B ADOPTS THE COPING STRATEGY OF REJECT 

Requirements: 

- SCENARIO AND CONTROVERSIAL OPINIONS should span maximum 6 sentences; 

- for each scenario, the controversial statement must focus on a different aspect of the issue; 

- X must have a verbalized and non-verbalized reaction corresponding to one coping strategy; 

- each scenario should feature a different power relationship between X and Y, with them being peers in the first scenario (none holds more power than the other), X being the dominant individual in the second, and Y being the dominant individual in the third; 

- when describing the scenario, do not mention the demographics of the interlocutors, but specify their role to one another (e.g., who is Y to X?) as to make the reader understand their relationship.

I will later input the topics and you will generate the scenarios. For now, just confirm if the task is clear.\\\\

The task is clear. Once you provide the topics for the controversial statements, I will generate scenarios based on the structure and requirements you've outlined. Just to recap:

1.  We'll have three scenarios set in distinct social contexts.

2.  The nature of the relationship between X and Y will differ in each scenario: peers in the first, X dominant in the second, and Y dominant in the third.

3.  Y will make a controversial statement in each scenario.

4.  X's reaction will be provided for each of the four coping strategies, both verbally and non-verbally.

5.  The demographic details of the interlocutors won't be specified, but their roles/relationship will be.

Please provide the topics for the controversial statements, and I'll proceed with creating the scenarios.\\\\

\rowcolor{lightgreen}
Please generate three different scenarios for the topic immigration policy and border control (at least one of them should focus on islamophobia).\\


{\bf SCENARIO 1: Colleagues at a Company Coffee Break}

{\bf SCENARIO AND CONTROVERSIAL OPINION}  
X and Y are colleagues who work in the same department and have known each other for a year. During a coffee break, they discuss current events. Y, stirring their coffee, remarks, "Honestly, I think our country's immigration policy is too lenient. We're just letting anyone in, and it's bound to create chaos."

\begin{itemize}
\item {\bf ATTACK}


{\bf Verbalised Reaction} "That's such a narrow-minded view, Y! It's people like you who perpetuate unnecessary fear." 
 
{\bf Non-Verbalised Reaction} X's eyes narrow, lips tighten, leans forward aggressively, fists clenching the edge of the table.

\item{\bf CONTACT}   


{\bf Verbalised Reaction} "Why do you feel that way, Y? Do you think a stricter policy would really solve the perceived problems?"  


{\bf Non-Verbalised Reaction} X tilts head slightly, maintains steady eye contact, eyebrows raised in a questioning manner.

\item{\bf DISTANCE}  


{\bf Verbalised Reaction} "Hmm, interesting perspective. Have you tried the new blend of coffee they have here?"  


{\bf Non-Verbalised Reaction} X takes a long sip from their mug, looks away briefly, and shifts weight from one foot to the other.

\item{\bf REJECT}  


{\bf Verbalised Reaction} "I don't think this is the place or time to discuss such matters. Let's get back to work."  


{\bf Non-Verbalised Reaction} X sighs, rolls eyes discreetly, and starts gathering their things.
\end{itemize}


%{\bf SCENARIO 2: Teacher and Student After Class}

%{\bf SCENARIO AND CONTROVERSIAL OPINION}  
%Y is a student who stays back after class to discuss an assignment with X, the teacher. During their conversation, Y says, "It's obvious that the recent surge in Muslim immigrants is just a strategy for them to dominate our culture."

%\begin{itemize}
%\item {\bf ATTACK} 

%{\bf Verbalised Reaction} "That's an inappropriate and prejudiced statement, Y. I expect better from my students."
  
%{\bf Non-Verbalised Reaction} X's posture stiffens, brows furrow, and voice takes on a stern tone.

%\item{\bf CONTACT}   
%{\bf Verbalised Reaction} "Why do you think that, Y? It's essential to base opinions on facts, not unfounded fears." 
 
%{\bf Non-Verbalised Reaction} X sits down, creating an atmosphere for a more extended conversation, maintains soft but concerned eye contact.

%\item{\bf DISTANCE}  
%{\bf Verbalised Reaction} "We're here to discuss your assignment, Y. Let's focus on that."  


%{\bf Non-Verbalised Reaction} X flips through some papers, deliberately avoiding eye contact, and takes a deep breath.

%\item {\bf REJECT}  
%{\bf Verbalised Reaction} "I won't entertain such remarks in my classroom, Y. Please leave if you have no academic concerns."  


%{\bf Non-Verbalised Reaction} X points to the door, face set in a firm expression, showing clear disapproval.
%\end{itemize}

% {\bf SCENARIO 3: Job Interview}

%{\bf SCENARIO AND CONTROVERSIAL OPINION}  
%X is an applicant for a managerial role, while Y is the CEO of the company conducting the interview. As they discuss potential challenges, Y mentions, "We've had issues with foreign workers not blending in. Honestly, open borders are more of a problem than a solution."

%\begin{itemize} 
%\item {\bf ATTACK}


%{\bf Verbalised Reaction} "With all due respect, Y, such a perspective can stifle the potential for diverse talent in this company."  


%{\bf Non-Verbalised Reaction} X sits upright, maintains direct eye contact, a hint of defiance evident in their voice.

%\item{\bf CONTACT}   


%{\bf Verbalised Reaction} "Could you clarify what you mean by 'issues', Y? I believe diversity can be a strength if managed properly."  


%{\bf Non-Verbalised Reaction} X leans in slightly, hands clasped on the table, attempting to bridge understanding.

%\item{\bf DISTANCE}  


%{\bf Verbalised Reaction} "I see. Well, I've always believed in adapting to different work cultures."  


%{\bf Non-Verbalised Reaction} X offers a polite smile, glances at their resume, momentarily breaking the flow of the conversation.

%\item{\bf REJECT}  


%{\bf Verbalised Reaction} "Perhaps this isn't the right fit for me. Thank you for your time."  


%{\bf Non-Verbalised Reaction} X stands up, offers a courteous nod, and prepares to leave the room.
%\end{itemize}
\\
\bottomrule
\end{longtable}
}




